Distance Restricted Manipulation in Voting

We introduce the notion of {\em Distance Restricted Manipulation}, where colluding manipulator(s) need to compute if there exist votes which make their preferred alternative win the election when their knowledge about the others' votes is a little inaccurate. We use the Kendall-Tau distance to model the manipulators' confidence in the non-manipulators' votes. To this end, we study this problem in two settings - one where the manipulators need to compute a manipulating vote that succeeds irrespective of perturbations in others' votes ({\em Distance Restricted Strong Manipulation}), and the second where the manipulators need to compute a manipulating vote that succeeds for at least one possible vote profile of the others ({\em Distance Restricted Weak Manipulation}). We show that {\em Distance Restricted Strong Manipulation} admits polynomial-time algorithms for every scoring rule, maximin, Bucklin, and simplified Bucklin voting rules for a single manipulator, and for the $k$-approval rule for any number of manipulators, but becomes intractable for the Copeland$^\alpha$ voting rule for every $\alpha\in[0,1]$ even for a single manipulator. In contrast, {\em Distance Restricted Weak Manipulation} is intractable for almost all the common voting rules, with the exception of the plurality rule. For a constant number of alternatives, we show that both the problems are polynomial-time solvable for every anonymous and efficient voting rule.

==> conclusion.tex <==
\section{Conclusion}

We have proposed a new model, called stable manipulation, of incorporating manipulator's uncertainty about others' preferences. Intuitively, in our model, the manipulator's uncertainty is distributed over the whole preference of other voters unlike many existing models in literature. We show that the stable manipulation problem usually admits polynomial time algorithms for the case of a single manipulator with the prominent exception of Copeland$^\alpha$ for $\alpha\in[0,1]$. We finally show, through simulation, that the probability of a random profile being stably manipulable drops drastically with a slight increase in the manipulator's uncertainty. Hence restricting any voter's information about the preferences of the others seems to be quite effective in hindering manipulation.
